Understanding Layered Portability from HPC to Cloud in Containerized Environments

Recent development in lightweight OS-level virtualization, containers, provides a potential solution for running HPC applications on the cloud platform. In this work, we focus on the impact of different layers in a containerized environment when migrating HPC containers from a dedicated HPC system to a cloud platform. On three ARM-based platforms, including the latest Nvidia Grace CPU, we use six representative HPC applications to characterize the impact of container virtualization, host OS and kernel, and rootless and privileged container execution. Our results indicate less than 4\% container overhead in DGEMM, miniMD, and XSBench, but 8\%-10\% overhead in FFT, HPCG, and Hypre. We also show that changing between the container execution modes results in negligible performance differences in the six applications.

==> backup.tex <==
\begin{table}[]
    \centering
    \caption{The impact of different layres in the chain of dependency}
    \begin{tabular}{c|c|c|c|c|c|}
     & Experiment A & Experiment B & Experiment C\\\hline
    Container Engine & \checkmark & \checkmark & rooless | root\\\hline
    application level library & \checkmark & BLAS | MPI | FFT & \checkmark\\\hline
    Compiler & \checkmark & \checkmark & \checkmark\\\hline
    system service & \checkmark & \checkmark & \checkmark\\\hline
    OS Kernel & \checkmark & \checkmark & \checkmark\\\hline
    HW & Neoverse N1 | N2 | APM X-GENE \t & \checkmark &\checkmark \\\hline
    \end{tabular}
    \label{tab:my_label}
\end{table}




\begin{table}[]
\centering
\begin{tabular}{|l|l|l|}
\hline
                      & \textbf{Sleipner (Host)}     & \textbf{Container (Image)} \\ \hline
\textbf{OS}           & Red Hat Enterprise Linux 9.3 & Rocky Linux 9.3            \\ \hline
\textbf{GCC Version}  & GCC 11.4                     & GCC 11.4                   \\ \hline
\textbf{MPI Version}  & Open MPI 5.0.2               & Open MPI 5.0.2             \\ \hline
\textbf{BLAS Version} & OpenBLAS 0.3.26              & OpenBLAS 0.3.26            \\ \hline
\end{tabular}
\caption{Software stack used at the Sleipner system, running Linux Kernel 5.14.0 and Docker 25.0.}
\label{tab:sleipner-software}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{|l|l|l|}
\hline
                      & \textbf{Pilot (Host)} & \textbf{Container (Image)} \\ \hline
\textbf{OS}           & OpenSUSE 15.5         & OpenSUSE 15.5              \\ \hline
\textbf{GCC Version}  & GCC 13.2              & GCC 13.2                   \\ \hline
\textbf{MPI Version}  & Open MPI 5.0.2        & Open MPI 5.0.2             \\ \hline
\textbf{BLAS Version} & OpenBLAS 0.3.26       & OpenBLAS 0.3.26            \\ \hline
\end{tabular}
\caption{Software stack used at the Pilot system, running Linux Kernel 5.14.21 and Podman 4.7.2.}
\label{tab:pilot-software}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{|l|l|l|}
\hline
                      & \textbf{CloudLab (Host)} & \textbf{Container (Image)} \\ \hline
\textbf{OS}           & Ubuntu 22.04             & Ubuntu 22.04         \\ \hline
\textbf{GCC Version}  & GCC 11.4                 & GCC 11.4                   \\ \hline
\textbf{MPI Version}  & Open MPI 5.0.2           & Open MPI 5.0.2             \\ \hline
\textbf{BLAS Version} & OpenBLAS 0.3.26          & OpenBLAS 0.3.26            \\ \hline
\end{tabular}
\caption{Software stack used at the CloudLab system, running Linux Kernel 5.14.21.}
\label{tab:cloudlab-software}
\end{table}

\begin{longtable}[c]{|c|c|c|}
\hline
\textbf{Application}     & \textbf{System Type} & \textbf{Parameters}                               \\ \hline
\endfirsthead
%
\endhead
%
\multirow{2}{*}{DGEMM}   & S1              & \textit{Size 5000 x 5000, 5 repeats}              \\ \cline{2-3} 
                         & S2              & \textit{Size 20000 x 20000, 5 repeats}            \\ \hline
\multirow{2}{*}{Hypre}   & S1              & \textit{Grid size (n) of 300}                     \\ \cline{2-3} 
                         & S2              & \textit{Grid size (n) of 3000}                    \\ \hline
\multirow{2}{*}{XSBench} & S1              & \textit{"Small" problem size}                            \\ \cline{2-3} 
                         & S2              & \textit{"Large" problem size}                            \\ \hline
\multirow{2}{*}{HPCG}    & S1              & \textit{Size 128, 128, 128}                       \\ \cline{2-3} 
                         & S2              & \textit{Size 256, 256, 256}                       \\ \hline
\multirow{2}{*}{MiniMD}  & S1              & \textit{400 iterations, size 64 64 64}            \\ \cline{2-3} 
                         & S2              & \textit{400 iterations, size 256 256 256}         \\ \hline
\multirow{2}{*}{fftMPI}  & S1              & \textit{100 iterations, grid 300 300 300, 3D FFT} \\ \cline{2-3} 
                         & S2              & \textit{150 iterations, grid 400 400 400, 3D FFT} \\ \hline
\caption{Parameters of the applications. All the parameters for the applications are the default ones if not stated here.}
\label{tab:parameters}\\
\end{longtable}


\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Name} & \textbf{CPU}                           & \textbf{Memory} & \textbf{Disk}          \\ \hline
m400          & 8x 64-bit Atlas/A57 cores @ 2.4 GHz    & 64GB ECC        & 120 GB of flash memory \\ \hline
Pilot         & 80x 64-bit Neoverse N1 cores @ 3.0 GHz & 526 GB          & 2.4TB SSD              \\ \hline
Sleipner      & 72x 64-bit Neoverse V2 cores @ 3.4 GHz & 592 GB          & 2.4TB SSD              \\ \hline
\end{tabular}
\caption{Infrastructure for the three systems used in this work.}
\label{tab:specs-infra}
\end{table}


\begin{figure}[!htb]
    \centering
    \begin{minipage}{.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/container-hirarchy.png}
        \caption{A hierarchical view of different layers in a containerized environment}
        \label{fig:hierarchy}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.63\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/image-flowchart.pdf}
        \caption{The main stages of building a image on a platform and deploying it on another platform.}
        \label{fig:stages}
    \end{minipage}
\end{figure}

